Fractional coloring of product signed graphs

This study examines the fractional chromatic number associated with the direct product of signed graphs. It shows that if $(H,\tau)$ is a signed circulant graph $G(n,S,T)$, then for any signed graph $(G,\sigma)$, the fractional chromatic number of their direct product is the lower number between the fractional chromatic number of $(G,\sigma)$ and $(H,\tau)$.

==> references.tex <==
@article{hedetniemi1966homomorphism,
  title={Homomorphisms of graphs and automata},
  author={Hedetniemi, Stephen T},
  journal={University of Michigan Technical Report},
  year={1966}
}

@article{shitov2019counterexample,
  title={Counterexamples to Hedetniemi's conjecture},
  author={Shitov, Yaroslav},
  journal={Annals of Mathematics},
  volume={190},
  number={2},
  pages={663--667},
  year={2019},
  publisher={JSTOR}
}

@article{zhu1992fractional,
  title={Fractional Hedetniemi's conjecture is true},
  author={Zhu, Xuding},
  journal={Journal of Combinatorial Theory, Series B},
  volume={55},
  number={1},
  pages={161--166},
  year={1992},
  publisher={Elsevier}
}

@article{harris2019fractional,
  title={Fractional coloring and the Hedetniemi-Lovász conjecture},
  author={Harris, David G},
  journal={SIAM Journal on Discrete Mathematics},
  volume={33},
  number={4},
  pages={2145--2160},
  year={2019},
  publisher={SIAM}
}

@article{harary1953notion,
  title={On the notion of balance of a signed graph},
  author={Harary, Frank},
  journal={Michigan Mathematical Journal},
  volume={2},
  number={2},
  pages={143--146},
  year={1953},
  publisher={University of Michigan}
}

@article{zaslavsky1982signed,
  title={Signed graph coloring},
  author={Zaslavsky, Thomas},
  journal={Discrete Mathematics},
  volume={39},
  number={2},
  pages={215--228},
  year={1982},
  publisher={Elsevier}
}

@article{máčajová2016fractional,
  title={Fractional coloring of signed graphs},
  author={Máčajová, Edita and Raspaud, André and Tardif, Claude},
  journal={European Journal of Combinatorics},
  volume={59},
  pages={1--13},
  year={2016},
  publisher={Elsevier}
}

@article{burr1976ramsey,
  title={On the Ramsey numbers of graphs},
  author={Burr, Stefan A and Erdős, Paul and Lovász, László},
  journal={Journal of Combinatorial Theory, Series B},
  volume={21},
  number={2},
  pages={111--114},
  year={1976},
  publisher={Elsevier}
}

